Sound Source Localization is All about Cross-Modal Alignment

Humans can easily perceive the direction of sound sources in a visual scene, termed sound source localization. Recent studies on learning-based sound source localization have mainly explored the problem from a localization perspective. However, prior arts and existing benchmarks do not account for a more important aspect of the problem, cross-modal semantic understanding, which is essential for genuine sound source localization. Cross-modal semantic understanding is important in understanding semantically mismatched audio-visual events, e.g., silent objects, or off-screen sounds. To account for this, we propose a cross-modal alignment task as a joint task with sound source localization to better learn the interaction between audio and visual modalities. Thereby, we achieve high localization performance with strong cross-modal semantic understanding. Our method outperforms the state-of-the-art approaches in both sound source localization and cross-modal retrieval. Our work suggests that jointly tackling both tasks is necessary to conquer genuine sound source localization.

==> template/def_custom.tex <==
% % % % % %
% % For IEEE journal version formatting
\usepackage{xspace}
\makeatletter
\def\onedot{\ifx\@let@token.\else.\null\fi\xspace}
\makeatother
% % % % % % %


\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.5}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother

\def\eg{\textit{e.g}\onedot} \def\Eg{{E.g}\onedot}
\def\ie{\textit{i.e}\onedot} \def\Ie{{I.e}\onedot}
\def\cf{\textit{c.f}\onedot} \def\Cf{{C.f}\onedot}
\def\etc{\textit{etc}\onedot} \def\vs{{vs}\onedot}
\def\wrt{\textit{w.r.t}\onedot} \def\dof{d.o.f\onedot}
\def\etal{\textit{et al}\onedot}



\newcommand{\Tref}[1]{Table~\ref{#1}}
\newcommand{\Eref}[1]{Eq.~(\ref{#1})}
\newcommand{\Fref}[1]{Figure~\ref{#1}}
\newcommand{\FCref}[1]{Chapter.~\ref{#1}}
\newcommand{\Cref}[1]{Chap.~\ref{#1}}
\newcommand{\Sref}[1]{Section~\ref{#1}}
\newcommand{\Aref}[1]{Alg.~\ref{#1}}

\newcommand{\R}{\mathbb{R}}
\newcommand{\matL}{\mathbf{Z}}
\newcommand{\matS}{\mathbf{E}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\Z}{\mathbf{Z}}

\newcommand{\CovX}{\mathbf{\Phi}}
\newcommand{\CovS}{\mathbf{\Gamma}}

\newcommand{\D}{\mathbf{D}}
\newcommand{\singularmat}{\Sigma}




\def\Vec#1{\mbox{\boldmath $#1$}}
\newcommand{\mO}{\mathbf{O}}
\newcommand{\mc}{\mathbf{c}}

\newcommand{\paragrp}[1]{\vspace{1mm}\noindent\textbf{#1}\,\,\,}

\newcommand{\oh}[1]{\textcolor{red}{Oh: {#1}}}
\newcommand{\kim}[1]{\textcolor{cyan}{Junsik: {#1}}}
\newcommand{\arda}[1]{\textcolor{blue}{#1}}
\newcommand{\gonhy}[1]{\textcolor{gray}{Gonhy: {#1}}}

\definecolor{steelblue}{rgb}{0.27, 0.51, 0.7}
\newcommand{\js}[1]{\textcolor{steelblue}{#1}}
